Building an Efficient Cluster Cosmology Software Package for Modeling Cluster Counts and Lensing

We introduce a software suite developed for galaxy cluster cosmological analysis with the Dark Energy Survey Data. Cosmological analyses based on galaxy cluster number counts and weak-lensing measurements need efficient software infrastructure to explore an increasingly large parameter space, and account for various cosmological and astrophysical effects. Our software package is designed to model the cluster observables in a wide-field optical survey, including galaxy cluster counts, their averaged weak-lensing masses, or the cluster's averaged weak-lensing radial signals. To ensure maximum efficiency, this software package is developed in C++ in the CosmoSIS software framework, making use of the CUBA integration library. We also implement a testing and validation scheme to ensure the quality of the package. We demonstrate the effectiveness of this development by applying the software to the Dark Energy Survey Year 1 galaxy cluster cosmological data sets, and acquired cosmological constraints that are consistent with the fiducial Dark Energy Survey analysis.

==> 04-philosophy.tex <==
% !TEX root = ms.tex

\subsection{Design Choices}

A crucial aspect in our software development is to deliver prediction code that can be implemented in a CosmoSIS \emph{module} for the likelihood calculation (Equation~\ref{eq:likelihood}), $\mu(\theta)$. 
We identify three challenges that we'd like to address during the development of the prediction code. 

First, the prediction of the cluster cosmological observables depend on a few models for different physics elements. Each of the models, for example the cluster mass-observable relation, halo mass function etc., is still under active development, and subject to activate updates. In addition, it is often desirable to explore several different forms of those models to assess the robustness of the analysis due to different physical assumptions.
%The examples are the models for the mass-observable relations and the halo mass function.
To make it as easier to change a model implementation, we decide to make the models modular, that one model implementation can be replaced by another that shares use of the same set of physical parameters. Each model is represented as a C++ class which is \emph{callable}, meaning that it implements the function call operator. We describe the details of this design in the next section.%Any model can thus be replaced with a different model that implements a function call operator with the same arguments. The C++ compiler will make sure that the number and types of the function arguments are the same; it is up to the physicist to make sure that the meanings of the arguments are the same. So, for example, each of our mass-observable relation classes can be called with three arguments: $\lt$, $\ln{M}$ and $\zt$, and wherever one of our mass-observable relations is used in a calculation, it could be replaced by a different one.

Second, the prediction of the summary statistics utilized in cluster cosmology analysis requires integrating over more than a few dimensions, as demonstrated in Section~\ref{s:theory}. The dimension of the integrals are often larger than two, and in the examples referenced in the previous section, reaches as many as eight. % Common integration tools such as those implemented in python, or GSL, have only implemented algorithms to handle 1-D or 2-D integrals. 
The dimension of those integrals can become even larger if future analyses becomes more complicated, for example by incorporating marginalization over parameters representing additional systematic effects. %Although it is possible to reduce the dimensionality of those integrals by using analytical forms or grouping independent variables into separate integral components, it is difficult to reduce the dimension of those integrals to one or two. 
Thus, an efficient integration method that can handle the number of dimensions in our integrals is need. We have found the algorithm in~\cite{Berntsen1991AnAA}, as implemented in the CUBA library~\cite{HAHN200578} to be the best currently available.

%Given these two challenges, our software design philosophy is to prioritize modularity and computing efficiency. Further, reproducibility of the code, achieved through testing, is held as a top priority together with modularity and efficiency. 

Thirdly, the integrals mentioned above need to be evaluated for each sample of cosmological parameters. If using Markov Chain Monte Carlo sampling, those integrals often need to be iterated $\sim 10^{6}$ times to evaluate the posterior distributions of cosmological parameters.
In order to finish the sampling in a reasonable timescale (ideally on a timescale of days), the integrals need to be performed very quickly. To help speed up the sampling process, CosmoSIS provides several samplers that can run in parallel, using multiple computer cores at the sample time in a single program. However, the scalability of the samplers are often limited to at most hundreds of ranks, and under-characterized even at such a parallelization scale. This is the reason that we have chosen to implement all our models and our integration routines in C++:
it provides the best combination of expressiveness and performance available. 

%Therefore it is critical for these calculations to be as computationally efficient as possible. 
%The time overhead of having the C implementation of the integration routine call back into the Python interpreter to evaluate the integrand would be much too great. For this reason, we chose to implement our integrand, and thus the models it contains, in a compiled language. We found that C++ provides features (notably classes and templates) that allowed us to write code that is both computationally efficient and maintainable. In the remainder of this section, we describe how we used these language features.


%We have developed the C++ infrastructure necessary to allow physicists without special expertise in numerical techniques to implement the calculations required for their physical models in an efficient fashion.



==> Makefile <==
all: ms.pdf

ms.pdf: ms.tex 01-intro.tex 02-theory.tex 03-parameter-estimation.tex \
	04-philosophy.tex 05-pipeline-structure.tex 06-testing-and-validation.tex \
	07-how-to-use.tex 08-discussion.tex 09-acks.tex mybibfile.bib
	latexmk -pdf ms.tex

clean:
	latexmk -C ms.tex
	rm -f ms.bbl ms.spl
	rm -f ms.pdf

view: ms.pdf
	open ms.pdf

